Vectorizing World Buildings: Planar Graph Reconstruction by Primitive Detection and Relationship Inference

This paper tackles a 2D architecture vectorization problem, whose task is to infer an outdoor building architecture as a 2D planar graph from a single RGB image. We provide a new benchmark with ground-truth annotations for 2,001 complex buildings across the cities of Atlanta, Paris, and Las Vegas. We also propose a novel algorithm utilizing 1) convolutional neural networks (CNNs) that detects geometric primitives and infers their relationships and 2) an integer programming (IP) that assembles the information into a 2D planar graph. While being a trivial task for human vision, the inference of a graph structure with an arbitrary topology is still an open problem for computer vision. Qualitative and quantitative evaluations demonstrate that our algorithm makes significant improvements over the current state-of-the-art, towards an intelligent system at the level of human perception. We will share code and data.

==> sections/10_results.tex <==
\section{Additional experimental results}
Figure \ref{fig:inter_results} presents intermediate results for detected primitives and relationships from our method. Figures \ref{fig:results_0}-\ref{fig:results_32} present additional experimental results against the five competing methods over all the testing samples.

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{images/inter_results.pdf}
\caption{Intermediate results displaying detected primitives and relationships in our pipeline.}
\label{fig:inter_results}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_0.png}
\caption{Additional qualitative results.}
\label{fig:results_0}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_1.png}
\caption{Additional qualitative results.}
\label{fig:results_1}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_2.png}
\caption{Additional qualitative results.}
\label{fig:results_2}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_3.png}
\caption{Additional qualitative results.}
\label{fig:results_3}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_4.png}
\caption{Additional qualitative results.}
\label{fig:results_4}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_5.png}
\caption{Additional qualitative results.}
\label{fig:results_5}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_6.png}
\caption{Additional qualitative results.}
\label{fig:results_6}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_7.png}
\caption{Additional qualitative results.}
\label{fig:results_7}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_8.png}
\caption{Additional qualitative results.}
\label{fig:results_8}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_9.png}
\caption{Additional qualitative results.}
\label{fig:results_9}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_10.png}
\caption{Additional qualitative results.}
\label{fig:results_10}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_11.png}
\caption{Additional qualitative results.}
\label{fig:results_11}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_12.png}
\caption{Additional qualitative results.}
\label{fig:results_12}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_13.png}
\caption{Additional qualitative results.}
\label{fig:results_13}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_14.png}
\caption{Additional qualitative results.}
\label{fig:results_14}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_15.png}
\caption{Additional qualitative results.}
\label{fig:results_15}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_16.png}
\caption{Additional qualitative results.}
\label{fig:results_16}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_17.png}
\caption{Additional qualitative results.}
\label{fig:results_17}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_18.png}
\caption{Additional qualitative results.}
\label{fig:results_18}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_19.png}
\caption{Additional qualitative results.}
\label{fig:results_19}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_20.png}
\caption{Additional qualitative results.}
\label{fig:results_20}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_21.png}
\caption{Additional qualitative results.}
\label{fig:results_21}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_22.png}
\caption{Additional qualitative results.}
\label{fig:results_22}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_23.png}
\caption{Additional qualitative results.}
\label{fig:results_23}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_24.png}
\caption{Additional qualitative results.}
\label{fig:results_24}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_25.png}
\caption{Additional qualitative results.}
\label{fig:results_25}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_26.png}
\caption{Additional qualitative results.}
\label{fig:results_26}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_27.png}
\caption{Additional qualitative results.}
\label{fig:results_27}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_28.png}
\caption{Additional qualitative results.}
\label{fig:results_28}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_29.png}
\caption{Additional qualitative results.}
\label{fig:results_29}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_30.png}
\caption{Additional qualitative results.}
\label{fig:results_30}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_31.png}
\caption{Additional qualitative results.}
\label{fig:results_31}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{results/grid_im_32.png}
\caption{Additional qualitative results.}
\label{fig:results_32}
\end{figure*}

==> sections/7_dataset.tex <==
\section{Benchmark statistics}
Figure \ref{fig:hist} shows histograms of training and testing samples against different numbers of corners, edges, and regions.
%for the numbers of corners, edges and regions in the training and testing samples.
%datasets, respectively.


\begin{figure}[!tb]
  \centering
  \includegraphics[width=\linewidth]{images/corners_hist.pdf}
  \includegraphics[width=\linewidth]{images/edges_hist.pdf}
  \includegraphics[width=\linewidth]{images/regions_hist.pdf}
  \caption{Building counts against the numbers of corners, edges, and regions.
  %Histograms of the numbers of corners, edges, and regions. Corners histogram. Number of buildings per number of corners contained in the training and testing dataset.
  }
  \label{fig:hist}
\end{figure}


\begin{comment}
\begin{figure*}[tb]
  \centering
  \includegraphics[width=\linewidth]{images/corners_hist.pdf}
  \caption{Corners histogram. Number of buildings per number of corners contained in the training and testing dataset.
  }
  \label{fig:corners_hist}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \includegraphics[width=\linewidth]{images/edges_hist.pdf}
  \caption{Edges histogram. Number of buildings per number of edges contained in the training and testing dataset.
  }
  \label{fig:edges_hist}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \includegraphics[width=\linewidth]{images/regions_hist.pdf}
  \caption{Regions histogram. Number of buildings per number of regions contained in the training and testing dataset.
  }
  \label{fig:regions_hist}
\end{figure*}
\end{comment}

==> sections/8_primitive_detector.tex <==
\section{Implementation details of primitive detectors}\label{primitive_detection}
Standard neural architectures are used for the primitive detection: Fully Convolutional Network (FCN) for corners \cite{wireframe_cvpr18}, Dilated Residual Networks (DRN) \cite{Yu2017DilatedRN} for edges, and Mask-RCNN \cite{he2017mask} for regions.


%Section \ref{primitive_detection} describes in more details the architectures utilized for primitives detection

\mysubsubsection{Corner detection} In our corner detection pipeline, we borrow an existing architecture~\cite{wireframe_cvpr18}. Our Fully Convolutional Network (FCN) divides the image in a $H_{b}\times W_{b}$ grid, where each cell is responsible for predicting a confidence score $c_{_{conf}}$ and $(x, y)$ coordinates of a corner residing within a bin. The corner network proposal head is trained using binary cross-entropy loss at each output cell in the grid. Similarly to \cite{wireframe_cvpr18}, we utilize a Google's Inception-v2 model \cite{szegedy2016rethinking} for encoding the input image. We train the network with a learning rate of $0.001$ (decay ratio $\gamma=0.1$ every each 5 epochs) using ADAM optimizer for 16 epochs and utilize only corners with $c_{_{conf}}\geq0.2$, batch size is set to 1. Our output grid size is $120\times120$ of 256-dimensional features which are regressed to the output of the network. 

\mysubsubsection{Edge detection} We utilize the DRN-D-105 architecture~\cite{Yu2017DilatedRN}. Given an input RGB image $I$ ($256\times256$), we obtain for each building an edge segmentation mask by optimizing a binary cross-entropy loss for each cell in the final feature map at the end of the network. We fine-tune the pre-trained DRN-D-105 architecture with learning rate equal to $0.0001$ for 40 epochs and batch size set to $8$. 

\mysubsubsection{Region detection} We utilize the official code release for Mask-RCNN \cite{he2017mask} for performing instance region segmentation. We train the network utilizing regions from the annotations as objects belonging to the same class. Our model was initialized with R-50-FPN architecture and trained with learning rate equal to $0.002$ with decay of $0.0001$. At test phase for a target building, we extract up to N (=100) regions.

==> sections/9_ip_formulation.tex <==
\section{Integer Programming (IP) formulation}\label{ip_formulation}

 %This and Section \ref{ip_formulation} provides additional details of our Integer Programming (IP) formulation.
 
\mysubsubsection{Objective function} 
Indicator variables are defined for each primitive: $I_{cor}$ for a corner $c\in\mathcal{C}$; $I_{edg}$ for an edge $e\in\mathcal{E}$; and $I_{reg}$ for a region $r\in\mathcal{R}$. We also have an indicator variable $I_{dir}$ for a corner to an incident edge direction relationship.
\begin{equation}\label{eqn:objective_function}
    \begin{split}
    %F(\mathcal{O}) = & \sum_{e \in \mathcal{E}}
    \max_{\{I_{cor},I_{edg},I_{reg},I_{dir}\}} & \sum_{e \in \mathcal{E}}\underbrace{(e_{_{conf}}c^{\prime}_{_{conf}} c^{\prime\prime}_{_{conf}}- 0.5^3)I_{edg}(e)}_{\mbox{corner and edge primitives}}   \\
        + 0.1& \sum_{c \in \mathcal{C}} \sum_{\theta \in \mathcal{D}_{c}} \underbrace{(\theta_{_{conf}} c_{_{conf}} - 0.5^2) I_{dir}(\theta, c)}_{\mbox{corner-to-edge relationship}} \\
        +&\sum_{r \in \mathcal{R}} \underbrace{I_{reg}(r)}_{\mbox{region primitive}}.
    \end{split}
\end{equation}
$c_{conf}$ and $e_{conf}$ denotes the confidence scores for the corner and the edge detections, respectively. $\theta_{conf}$ denotes the corner-to-edge relationship confidence.
Note that region and region-to-region relationship confidences were used for thresholding the detections and will not be in the optimization. With abuse of notation, $c^{\prime}$ and $c^{\prime\prime}$ denotes the end-points of an edge $e$.

\mysubsubsection{Slack Variables}
In the following sections we describe constraints as hard constraints however, we utilize slack variables to soften them. For instance, given a constraint in the form of $I_A I_B = C$, we can split it into two additional constraints $I_A I_B \leq C + S_{up}$ and $I_A I_B \geq C-S_{lo}$ and add $-S_{up}$ and $-S_{lo}$ in the objective function, in order to approximate a lower and upper bound to a constant $C$. We perform similar procedure for constraints in the form of $I_A I_B \geq C$ and $I_A I_B \leq C$.

\mysubsubsection{Topology constraints}
    We enforce three topology priors as constraints: (1) active edge must have its end-points active (Eq. ~\ref{eq:topology_1}), (2) degree of each corner should be greater or equal to two (Eq. ~\ref{eq:topology_2}) and (3) two intersecting edges $e_{k}$ and $e_{l}$ can not be active at the same time (Eq. ~\ref{eq:topology_3}).   
    \begin{align}
        &\sum_{e \in \mathcal{E}_c}I_{edg}(e)\geq 2I_{cor}(c)\label{eq:topology_1},\\
        &I_{cor}(c^{\prime}) + I_{cor}(c^{\prime\prime})= I_{edg}(e)\label{eq:topology_2},\\
        &I_{edg}(e_{k})I_{edg}(e_{l})= 0\label{eq:topology_3},
    \end{align}
    where $\mathcal{E}_c$ represents the set of all candidate edges incident to $c$.
    
\mysubsubsection{Region primitive constraints} 
    Region primitives are added as constraints by (1) enforcing indicator variables of intersecting edges and regions to not be active at the same time (Eq. \ref{eq:region_intersection}) and (2) enforcing the activation of edge indicator variables surrounding a region (Eq. \ref{eq:region_boundary}). For the latter, we trace a boundary of the predicted region and cast rays $\gamma$ (i.e. line segments with length and width equal to 100 and 2 pixels, respectively) in the outward direction (i.e. normal to the traced boundary) for every 2 pixels. We collect edges that intersect a $\gamma$ and enforce that at least one edge should be active. 
    
    \begin{align}
        \sum_{e \in \mathcal{E}^{r}} I_{edg}(e)&I_{reg}(r) = 0,\label{eq:region_intersection}\\
        \sum_{e \in \mathcal{E}^{\gamma}} I_{edg}(e)& \ge I_{reg}(r),\label{eq:region_boundary}
    \end{align}
    where $\mathcal{E}^{r}$ and $\mathcal{E}^{\gamma}$ are the set of edges that intersect a region $r$ and a ray $\gamma$, respectively.
    
\mysubsubsection{Region-to-region relationship constraints} 
    Considering a pair of regions sharing a common boundary predicted as a segmentation mask. We fit a line segment to the boundary segment, consider an orthogonal line segment $\beta$ (16 pixels in length) at the center. We collect all the edge primitives that intersect with the last line segment. One of them must be the boundary edge.
    \begin{align}
    \sum_{e \in \mathcal{E}^{\beta}} I_{edg}(e) &= 1\label{eq:region_region},\\
    \end{align}
    where $\mathcal{E}^{\beta}$ represents the set of all candidate edges intersecting $\beta$.
    
\mysubsubsection{Corner-to-edge relationship constraints} 
    We design constraints to enforce incident edge indicator variables to be active consistently with its corresponding corner and directional bin. In addition, if a corner-to-edge confidence is below 0.2 for a corner and an incident direction, we do not allow any edges in that direction bin to be on. In order to achieve this the following two constraints are sufficient.
    \begin{align}
        \sum_{e \in \mathcal{E}^{\theta}} I_{edg}(e) &= I_{dir}(\theta, c)\label{eq:junction_constraint_1},\\
        \sum_{e \in \mathcal{E'}} I_{edg}(e)&= 0\label{eq:junction_constraint_2},\\
    \end{align}
    where $\mathcal{E}^{\theta}$ is a set of collected edges in a direction $\theta$ within 5 degrees in angular distance and $\mathcal{E'}$ is a set of edges incident in all directions with confidence lower than 0.2.


% 	\item $S_\theta(\theta_j) \ge 0$, for junction directions $\theta_j$,
% 	\item $S^{lo}_c(e) \ge 0$, for edges $e$,
% 	\item $S^{up}_c(e) \ge 0$, for edges $e$,
% 	\item $S^{lo}_r(e) \ge 0$, for edges $e$,
% 	\item $S^{up}_r(e) \ge 0$, for edges $e$,

% where $\theta_j$ and $e$ are predicted directions at each junction $j$ and candidate edges, respectively. Also, $S_\theta(\theta_j)$, $S^{lo}_c(e)$ and $S^{up}_c(e)$, $S^{lo}_r(e)$ and $S^{up}_r(e)$ are integer slack variables for violating predicted junction directions, closed polygons for regions and boundaries between adjacent regions, respectively.


% where $\lambda_e$, $\lambda_j$ and $\lambda_r$ weight the influence of input signals for edge map, junction estimation and region instance segmentation. In addition, $\lambda_{s_\theta}$, $\lambda_{s^{lo}_c}$, $\lambda_{s^{up}_c}$, $\lambda_{s^{lo}_r}$ and $\lambda_{s^{up}_r}$ are weights for violating their corresponding constraints. 

% \textbf{Junction constraints.} We first describe three constraints for including junction predictions in the IP formulation. Here we constrain active junctions (i.e. $J(j)=1$) to connect with only one edge at each active direction (i.e. $\Theta(\theta_j)=1$) within a certain error margin $\delta$ (=5) in degrees. Thus, given a direction $\theta_j$ for a certain junction $j$, we collect a set of incident edges ($\mathcal{E}_{\theta}$) within $\delta$ degrees and select only one edge if the indicator variable $\Theta(\theta_j)$ is active (Eq. \ref{eq:junction_constraint_1}). The second junction constraint prohibits incident edges to be active in non predicted directions, however we soften this constraint by including a slack variable $S_\theta(\theta_j)$ (Eq. \ref{eq:junction_constraint_2}), in order to allow incident edges in wrong directions, in case other input sources (i.e. edge and region information) encourage to do so. Thus, let $\mathcal{E'}_j$ be set of incident edges not contained in any direction $\theta$, we can write Eq. \ref{eq:junction_constraint_2}. In addition, we constrain the degree of each junction to be at least two in case the junction is active ($J(j)=1$), therefore, the sum of all incident edges for each junction should be greater of equal to two. Considering that $\mathcal{E}_j$ is the set containing all incident edges for a junction $j$, we can write this constraint as in Eq. \ref{eq:junction_constraint_3}, as a result this guarantees closed polygons in the output graph. All three constraints are formulated as follows:

% \begin{align}
% \sum_{e \in \mathcal{E}^{\theta}_j} E(e) &= \Theta(\theta_j)\label{eq:junction_constraint_1},\\
% \sum_{e \in \mathcal{E'}_j} E(e)&= S_\theta(\theta_j)\label{eq:junction_constraint_2},\\
% \sum_{e \in \mathcal{E}_j}E(e)&J(j)\geq 2J(j).\label{eq:junction_constraint_3}
% \end{align}

% Note that the first constraint is defined per direction at each junction, while the second and third constraints are defined per junction.

% \textbf{Connectivity constraint.} Junctions and edges indicator variables must be consistent with the connections in the topological graph of the building, in order to avoid invalid configurations of active junctions and edges. For instance, consider two active junctions $j_k$ and $j_l$ (i.e. $J(j_k)=1$ and $J(j_l)=1$), if the edge connecting $e(j_k, j_l)$ is active then the indicator variables for $j_k$ and $j_l$ must be active. The same inconsistent configuration may happen from the junction perspective, if $j_k$ is not active (i.e. $J(j_k)=0$), then incident edges to $j_k$ must be deactivated. We translate this constraint in the following equation: 

% \begin{align}\label{eqn:connectivity}
% (J(j_k) + J(j_l) - 2) E(e(j_k, j_l)) &= 0.
% \end{align}

% This constraint is defined for each edge $e$ and is required when junction variables $J(j)$ are included in the formulation, in order to keep connectivity consistency between junctions and edges. The inclusion of junction indicator variables is particularly important considering that we want to suppress false alarm junction detections (i.e. junction degree equal to zero, when $J(j)=0$) and enforce a minimum degree at each junction (i.e. Eq. \ref{eq:junction_constraint_3}, when $J(j)=1$), simultaneously, which is normally necessary in practice.

% \textbf{Region constraints.} Equipped with MaskRCNN region detections $r$ and its contour defined by a set of points $\mathcal{C}^r$. We enforce five constraints that utilizes region masks directly in the IP formulation for obeying the following three conditions: a region should be bounded by edges, intersecting edges and regions should not coexist and adjacent regions should be bounded by only one edge. 

% In order to enforce the first condition, we derive two constraints that specify a lower and upper bound for the number of candidate edges lying on the boundary around each region $r$. Considering a region $r$ is always surrounded by edges, there must be at least one edge in any direction outwards $r$. We utilize a simple heuristic for selecting candidate edges at each direction, which consists of casting a ray $\gamma$ from each point ($p^r \in \mathcal{C}^r$) in the contour outwards $r$. Let $\mathcal{E}^\gamma$ be set of edges intersected by ray $\gamma$ from a point $p^r$ in contour $\mathcal{C}^r$, for each point $p^r$ we can enforce a lower bound $|\mathcal{E}^\gamma| \ge 1 - S^{lo}_c(e)$ (i.e. Eq. \ref{eq:region_constraint_lower}). In addition, in case ray $\gamma$ does not intersect any other region nor $r$, the upper bound constraint is defined as $|\mathcal{E}^\gamma| \le 1 + S^{up}_c(e)$ (i.e. Eq. \ref{eq:region_constraint_upper}). $S^{lo}_c(e)$ and $S^{up}_c(e)$ are slack variables to soften the constraints. The lower and upper bound constraints can be written as follows:

% \begin{align}
% \sum_{e \in \mathcal{E}^{\gamma}} E(e)R(r) &\ge R(r) -S^{lo}_c(e)\label{eq:region_constraint_lower},\\
% \sum_{e \in \mathcal{E}^{\gamma}} E(e)R(r) &\le R(r) + S^{up}_c(e)\label{eq:region_constraint_upper}.
% \end{align}

% From the second condition, we can directly derive a mutually exclusive constraint between intersecting edges and regions. We define an intersection between an edge $e$ and a region $r$ by rasterizing $e$ with width equal to 4 pixels and calculating the percentage of overlap of $e$ in $r$. We consider an edge overlapping a region by over 10\% as an intersection. Let $\mathcal{E}^{\phi}$ be the set of edges that intersects a region $r$, we can write the following constraint for each $r$.

% \begin{align}
% \sum_{e \in \mathcal{E}^{\phi}} E(e)R(r) &= 0\label{eq:region_constraint_intersection}.
% \end{align}

% In the third condition, we want to constrain the number of edges lying on the shared boundary between adjacent regions. Again we select the set of candidate edges lying on the shared boundary between region $r$ and its adjacent regions by casting rays outwards $r$ from its contour points. For each contour point $p^r$, we cast a ray $\beta$ outwards $r$ for checking intersection with adjacent regions. We collect a set of edges $\mathcal{E}^{\beta}$ between $p^r$ and the closest point of intersection $p^{r'}$ of $\beta$ with another region $r'$ and enforce an lower bound ($|E|\ge1-S^{lo}_c(e)$) and an upper bound constraint ($|E|\le1+S^{up}_c(e)$) (i.e. Eqs. \ref{eq:region_constraint_inter_region_lower} and \ref{eq:region_constraint_inter_region_upper}), in case $R(r)$ is an active region. Therefore, the constraints can be written as follows:   


% where $S^{lo}_c(e)$ and $S^{up}_c(e)$ are slack variables to soften the lower and upper bound constraints. It is worth mentioning that we just include these constraints in case ray $\beta$ intersects another region and there is no self intersection with region $r$ nor with the area outside the building footprint (background), which can be estimated by accumulating all detected region segments from MaskRCNN. Therefore, these constraints are defined per  point in the contour (i.e. for each $p^r \in \mathcal{C}^r$) under the conditions mentioned before. In addition, Eqs. \ref{eq:region_constraint_inter_region_lower} and \ref{eq:region_constraint_inter_region_upper} are simplified to ignore if the intersected region $r'$ is active, in order to avoid higher order terms in the constraint. 

% \textbf{Objective function.} We breakdown the objective function of our IP formulation in four terms: 1) Sum of edge indicator variables ($E(e)$) weighted by junction ($c^j$) and edge confidence scores ($c^{e}$) minus a constant $\tau_j$ (=0.125). 2) Sum of junction directions indicator variables ($\Theta(\theta_j)$) weighted by junction and its directions confidence scores, $c^j$ and $c^{\theta}$, respectively, minus a constant $\tau_\theta$. 3) Sum of region indicator variables ($R(r)$) 4) Minus sum of slack variables (i.e. $S_\theta(\theta_j)$, $S^{lo}_c(e)$, $S^{up}_c(e)$, $S^{lo}_r(e)$ and $S^{up}_r(e)$). Considering $\mathcal{O}$ is the set containing all indicator and slack variables, we combine the four terms mentioned before and write the equation for the objective function $F(\mathcal{O})$, as follows:


